Massively Digitized Power Grid: Opportunities and Challenges of Use-inspired AI

This article presents a use-inspired perspective of the opportunities and challenges in a massively digitized power grid. It argues that the intricate interplay of data availability, computing capability, and artificial intelligence (AI) algorithm development are the three key factors driving the adoption of digitized solutions in the power grid. The impact of these three factors on critical functions of power system operation and planning practices are reviewed and illustrated with industrial practice case studies. Open challenges and research opportunities for data, computing, and AI algorithms are articulated within the context of the power industry's tremendous decarbonization efforts.

==> sec/2_AI_progress.tex <==
\section{Recent Progress in Artificial Intelligence}
The proliferation of AI has made groundbreaking accomplishments in a variety of domains in recent years. Such unprecedented success is attributed to three factors, massively available data, massively improved computing performance, and massively improved AI algorithms~\cite{bertsunas_youtube,openai}. 

%%%%%%%%%%%%% Data %%%%%%%%%%%%%%%%%
Data of large volume and heterogeneous structure have been generated at an unprecedented rate from diverse resources since 2010~\cite{oussous2018big,faroukhi2020big,agrahari2017review}, such as Internet of Things (IoT) records, social media, smart devices, health systems, and so on. The availability of tremendous data has enabled applications of valuable knowledge extraction in industry sectors fields~\cite{national2013frontiers} spanning manufacturing~\cite{hilbert2016big}, healthcare~\cite{dimitrov2016medical}, government~\cite{pencheva2020big}, retail~\cite{einav2014economics}, infrastructure~\cite{chen2016promises,zhou2016big,baccarelli2016energy}, and etc.
% which is estimated 400 billion gigabytes in total by 2020.
Particularly, numerous open-source high-quality training datasets~\cite{wikipedia_datasets}, thanks to researchers, have been created to boost AI research in the aspects of model training, test, calibration, and benchmark.
% The internet of things (IoT) is enabling the collection of exabytes of text, voice, image and other forms of training data for AI models.

%%%%%%%%%%%%% Computing %%%%%%%%%%%%%%%%%
The remarkable improvement in computing performance is another key factor of the proliferation of AI, credited to advances in hardware, software, and generic algorithms~\cite{leiserson2020there}. It has enabled a variety of practical large-scale AI models, of which the amount of computation for model training has been increasing exponentially with a 3.4-month doubling period~\cite{openai,thompson2020computational}.
% For instance, the total speedup of solving mixed integer optimizations (MIO) in the 25 years between 1991 and 2016 is 2.2 trillion times~\cite{bertsunas_youtube}, of which a factor of 1.6 million is due to hardware speedup from 59.7 GFlop/s in 1993 to 93.0 PFlop/s in 2016, while another factor of 1.4 million is due to software and algorithmic speedup from CPLEX 1.2 in 1991 to Gurobi 6.5 in 2015.
% Computing: hardware
The rapid progress of hardware computing resources dominantly have been driving the development of AI models. Of particular note, the emergence of generic purpose graphic processing units (GPUs)~\cite{NVIDIA_V100} and AI accelerator application-specific integrated circuit (ASIC) such as~\cite{google_TPU,merolla2014million,graphcore_ipu,nvidia_MCU} can accelerate AI model training dramatically.
% Computing: software
In addition, AI-tailored software has been developed to exploit hardware computing resources~\cite{capra2020hardware}. For instance, basic linear algebra subroutines (BLAS)  libraries~\cite{lawson1979algorithm,dongarra1990algorithm,golub2012matrix,AMD_LibM,Intel_MKL,Nvidia_cuBLAS} have been created to optimize common linear algebra operations that are recursively executed in deep neural networks. Particularly, NVIDIA GPUs, which are widely supported by mainstream deep learning framework~\cite{abadi2016tensorflow,jia2014caffe,paszke2017automatic}, have a highly optimized library cuDNN~\cite{Nvidia_cuDNN} enabling high-performance GPU acceleration.
% Computing: generic algorithms
The progress of generic algorithms has also improved computing performance, exhibiting enormous heterogeneity on problems of different types and sizes~\cite{sherry2021point}. It is worth noting that some large-size problems benefit equally or even more from algorithmic improvement than from Moore's law. 
For instance, the total speedup of solving mixed integer optimizations (MIO) is 2.2 trillion times during the 25 years between 1991 and 2016~\cite{bertsunas_youtube}, of which a factor of 1.6 million is due to hardware speedup from 59.7 GFlop/s in 1993 to 93.0 PFlop/s in 2016, while another factor of 1.4 million is due to software and algorithmic speedup from CPLEX 1.2 in 1991 to Gurobi 6.5 in 2015.
% To demonstrate the contribution of algorithmic improvement to overall computing improvement, we illustrate linear programming (LP) and mixed integer optimizations (MIO) as examples, which are commonly used to solve many ML and statistics problems. The computational performance of LP in the 15 year between 1988 and 2003 is improved by 43 million times~\cite{PCAST2010designing}, of which a factor of 1000 is due to processor speedup while another factor of 43000 is due to improvements in algorithms.The total speedup of solving MIO in the 25 years between 1991 and 2016 is 2.2 trillion times~\cite{bertsunas_youtube}, of which a factor of 1.6 million is due to hardware speedup from 59.7 GFlop/s in 1993 to 93.0 PFlop/s in 2016, while a factor of 1.4 million is due to software speedup from CPLEX 1.2 in 1991 to Gurobi 6.5 in 2015.

%%%%%%%%%%%%% AI algorithm %%%%%%%%%%%%%%%%%
With the fast-growing AI infrastructure that provides massive data and computing capacity, numerous advanced AI algorithms have been developed in the past decade. State-of-the-art performance on benchmark datasets for tasks of multiple research fields has had continued improvement by pre-trained models~\cite{yang2019xlnet,devlin2018bert,szegedy2017inception,radford2018improving} and novel AI model architecture such as AlexNet~\cite{krizhevsky2012imagenet}, VGG~\cite{simonyan2014very}, ResNet~\cite{he2016deep}, Transformer~\cite{vaswani2017attention}, and etc. Attributed to industry-led investment and contribution, AI applications have also emerged in a variety of domains~\cite{ai100_2021}, including but not limited to language processing~\cite{qiu2020pre}, speech recognition~\cite{nassif2019speech}, facial recognition~\cite{facial_recognization}, real-time object detection~\cite{redmon2018yolov3}, multiplayer game~\cite{vinyals2019grandmaster,silver2017mastering,silver2018general}, recommendation system~\cite{zhang2021artificial}, intelligent robotics~\cite{boston_dynamics_spot,boston_dynamics_atlas,agility_robotics}, driving assistant system~\cite{tesla_autopilot}, disease diagnosis~\cite{rajpurkar2017chexnet}, drug discovery~\cite{paul2021artificial}, finance~\cite{wu2020towards}, and so on.

Electric power sector has involved in such tide of revolutionary digitization and AI-ization that cultivates new functions and applications. In the following sections, we will introduce the advancement of AI infrastructure in digitized power grids and then elaborate AI algorithm-based approaches and industry use cases that address the arising challenges of modern power grids towards decarbonization.
% \section{Data-driven Technology Enabled by Digitization in Power Systems}
